Point defects in IBS coating for very low loss mirrors

High reflective coatings are used in many physics experiments. Despite the high quality of the opticalcoating, the performances of the mirrors is altered by the scattered light induced by micrometers sizedefects in the coating layers. The topic of this paper is the study of the point-like scatterers present in thespecific coating of the mirrors used in state of the art, high sensitivity optical experiments. We studied thebehavior of the materials according to different thicknesses, and how the defects change after annealing.To our knowledge, this is a first insight into the formation of such defects for different materials andthickness and how this is reduced when samples are annealed.

==> param.tex <==
%%%% define title aspects %%%%
\def\titlefont{\normalfont\LARGE\bfseries}  %% insurance
\def\title#1{\gdef\@title{\titlefont #1}} 

\def\settitlefont{
%%% identify font used; cmr = Computer Modern Roman, ptm = Times Roman
\typeout{\rmdefault -font_in_spiecls}
\def\cmr{cmr}  % variables for font tests
\newif\ifcmr
\def\ptm{ptm}
\newif\ifptm
\ifthenelse{\equal{\rmdefault}{\cmr}}{\cmrtrue}{\cmrfalse}
\ifthenelse{\equal{\rmdefault}{\ptm}}{\ptmtrue}{\ptmfalse}
%%% scale title according to default font and size
\if0\@ptsize    % 10pt text; use 16pt bold fonts
  \renewcommand{\titlefont}{\fontsize{16pt}{19.2pt}\selectfont\bfseries}
  \ifcmr  \font\titlefont = cmbx12 at 16truept  \fi
\fi
% for 11pt text, title font should be 17pt = \LARGE for 11pt. No change needed
\if2\@ptsize    % 12pt text; use 19.2pt bold fonts
  \renewcommand{\titlefont}{\fontsize{19.2pt}{23pt}\selectfont\bfseries}
  \ifcmr  \font\titlefont = cmbx12 at 19.2truept  \fi
\fi  } 

\def\authorinfo#1{\gdef\@authorinfo{#1}}
\authorinfo{}     %% default is empty
%\let\@affiliation\@empty
%\def\affiliation#1{\gdef\@affiliation{#1}}

% Set special footnote indentation for authorinfo
\renewcommand\@makefntext[1]{\leftskip=1.4em\hskip-0em\@makefnmark#1}

